Towards Scene Graph Anticipation

Spatio-temporal scene graphs represent interactions in a video by decomposing scenes into individual objects and their pair-wise temporal relationships. Long-term anticipation of the fine-grained pair-wise relationships between objects is a challenging problem. To this end, we introduce the task of Scene Graph Anticipation (SGA). We adapt state-of-the-art scene graph generation methods as baselines to anticipate future pair-wise relationships between objects and propose a novel approach SceneSayer. In SceneSayer, we leverage object-centric representations of relationships to reason about the observed video frames and model the evolution of relationships between objects. We take a continuous time perspective and model the latent dynamics of the evolution of object interactions using concepts of NeuralODE and NeuralSDE, respectively. We infer representations of future relationships by solving an Ordinary Differential Equation and a Stochastic Differential Equation, respectively. Extensive experimentation on the Action Genome dataset validates the efficacy of the proposed methods.

==> paper_tex_files/backup.tex <==

\eat{
As there is currently no established baseline model for the task of Scene Graph Anticipation, we propose various adaptations of Dynamic Scene Graph models to serve as a foundational framework for anticipation in this context. In this research context, we leverage Scene Graph models as a fundamental framework for anticipation. We modify the established Dynamic Scene Graph generation models, STTran\cite{cong_et_al_sttran_2021} and DSGDetr\cite{Feng_2021} for the anticipation task. Our adaptations, namely STTran+, STTran++, DSGDetr+, and DSGDetr++, serve as the proposed foundational framework for this endeavor.
\\
In the STTran+ and DSGDetr+ methodologies, we adapt their temporal relationship transformers into auto-regressive anticipation transformers. These transformers are trained to forecast future relationships between subject-object pairs depicted within the provided contextual frames. In the STTran++ and DSGDetr++ methodologies, we employ two distinct temporal transformers: the Temporal Context Encoder and the Anticipatory Encoder. The Temporal Context Encoder is responsible for encoding the temporal relationships among subject-object pairs and producing the scene graph of the provided context frames. The Anticipatory Encoder, built upon the Temporal Context Encoder, utilizes the relationship latents generated by the context encoder as input to predict future relationship latents for the same subject-object pairs. The architectural framework for both + and ++ models is shown in Fig \ref{fig:method_pipeline}.
}

